Video Denoising in Fluorescence Guided Surgery

Fluorescence guided surgery (FGS) is a promising surgical technique that gives surgeons a unique view of tissue that is used to guide their practice by delineating tissue types and diseased areas. As new fluorescent contrast agents are developed that have low fluorescent photon yields, it becomes increasingly important to develop computational models to allow FGS systems to maintain good video quality in real time environments. To further complicate this task, FGS has a difficult bias noise term from laser leakage light (LLL) that represents unfiltered excitation light that can be on the order of the fluorescent signal. Most conventional video denoising methods focus on zero mean noise, and non-causal processing, both of which are violated in FGS. Luckily in FGS, often a co-located reference video is also captured which we use to simulate the LLL and assist in the denoising processes. In this work, we propose an accurate noise simulation pipeline that includes LLL and propose three baseline deep learning based algorithms for FGS video denoising.

==> sec/2_related.tex <==
\section{Related Works:}

\noindent\textbf{Image Denoising: }Recent deep learning methods for image denoising have attained strong performance~\cite{zhang2023kbnet,chen2022simple,zamir2022restormer,zamir2021multi,chen2021hinet,wang2022uformer,tu2022maxim,cheng2021nbnet,zamir2020learning}. Many of these methods modify the standard U-Net architecture~\cite{unet} by adding, for example, attention mechanisms~\cite{wang2022uformer,zamir2022restormer,tu2022maxim,cheng2021nbnet},  normalization~\cite{chen2021hinet}, or kernel bases~\cite{zhang2023kbnet} to increase the ability for networks to aggregate spatial information. NAFnet~\cite{chen2022simple} is a state of the art image denoiser which combines key elements of other image denoisers with a goal of simplifying the core architecture resulting in a light weight network with strong performance. NAFnet uses a simplified channel attention~\cite{hu2018squeeze} for global information aggregation, depth wise convolutions~\cite{han2021demystifying,liu2022convnet} for local information, layer normalization~\cite{ba2016layer} to stabilize training and "Simple Gate" as the non-linearity. We find NAFnet works well for our problem with fast training times, so we use it as the primary network backbone for our baseline methods.



\noindent\textbf{Video Denoising: } The temporal information in video can be quite useful to denoising tasks; however, the additional dimension can come with computation and memory costs so dealing with the time dimension efficiently is a key problem in video denoising. Each temporal strategy has many approaches; however, in this work we are dealing with a new problem with a domain shift and it would be impractical to update all methods to properly use the RV, force causality, and retrain all methods on our dataset. Instead we choose one of best performing methods to modify and retrain from each category for comparison with our new baseline models. 

We broadly categorize the temporal processing strategies into three categories.The first temporal approach is \textbf{sliding window} strategies~\cite{tassano2019dvdnet,BP-EVD,Tassano_2020_CVPR,wang2019edvr,yue2020supervised,qi2022real,van2021real} which have a fixed temporal receptive field that is sequentially moved throughout the video sequence. BP-EVD~\cite{BP-EVD} and FastDVDNet\cite{Tassano_2020_CVPR} rely on a cascaded approach where successive frames are grouped together as inputs into an initial block whose outputs are later fused with the outputs of temporally adjacent blocks. We choose to use FastDVDNet as the baseline model for this category because it has strong denoising performance and it's structure easily lends itself to a causal implementation. The second strategy is based on \textbf{Recurrent Neural Networks} (RNNs)~\cite{huang2015bidirectional,maggioni2021efficient,chan2021basicvsr,chan2022basicvsr++,cao2023learning,xiang2022remonet,chen2016deep}. Recurrent neural networks (RNNs) can pass information forward and backward in time recursively throughout many frames of video, in principle allowing for very long range temporal aggregation. We choose to use BasicVSR++~\cite{chan2022basicvsr++} to represent the RNN category. BasicVSR++ uses a grid propagation strategy based on flow guided~\cite{chan2021understanding} deformable convolutions~\cite{dai2017deformable,zhu2019deformable} with second order connections that allow features to be aligned, aggregated and propagated in time to achieve state of the art performance on video denoising~\cite{chan2022generalization}. The third temporal strategy are \textbf{Align and Merge} (A\&M) methods~\cite{Arias2017VideoDV,VBM4D,hasinoff2016burst,xu2020learning,davy2018non,vaksman2021patch,seets2023ofdvdnet,tang2023automated}. A\&M strategies in deep learning are extensions of block~\cite{Arias2017VideoDV,VBM4D} or patch matching~\cite{hasinoff2016burst} non-learning based methods. These strategies rely on combining multiple observations of the same object across time to reduce noise variance. These methods align or match regions of the video to deal with motion and then combine these matched regions in a merge step to denoise the video. OFDVDnet~\cite{seets2023ofdvdnet} was developed for FGS denoising and uses an explicit align and merge step to aggregate many frames of temporal information to be used as input into downstream CNN without increasing the memory requirements of training large temporal receptive fields. OFDVDnet also demonstrated the importance of the inclusion of the RV for both alignment and additional spatial information in the FGS denoising process.

While transformer architectures~\cite{dosovitskiy2020image,carion2020end,fan2021multiscale} may offer another temporal approach, we note that in video restoration tasks transformer architectures lack causality and are meant to be used on a video-to-video or clip-to-clip basis~\cite{liang2022rvrt,liang2022vrt}. In terms of performance CNN based methods, such as NAFnet or BasicVSR++, perform comparably to transformer architectures in denoising tasks.With this in mind and to reduce complexity of our baseline models we choose to focus on CNN based architectures in this work.

\noindent\textbf{Contrast Agent Outlook}
Currently in the clinic, non-targeted drugs are commonly used; the most popular is indocynanine green (ICG) which is most used in tissue perfusion~\cite{komorowska2010intraoperative,yoshimatsu2021application} and lymph node~\cite{Kitai2005} targeting applications but has limited utility in other surgical operations such as tumor targeting due to low specificity~\cite{Zhang2017}. Expanding the use of FGS to other surgeries require creating new contrast agents; however, this is an expensive process not helped by the fact that acceptable agents have tight constraints~\cite{Zhang2017} on signal levels, the stokes shift~\cite{lakowicz2006principles}, specificity, and photo-bleaching to ensure hardware devices can produce a useful real-time video. For example, one promising contrast agent is the naturally occurring auto-fluorescence~\cite{betz1999autofluorescence,demos2004near} or that auto-fluorescent lifetimes~\cite{marcu2012fluorescence,weyers2022intraoperative} have been proposed to deal with low specificity of cancer targeting drugs~\cite{belykh2018optical,alfonso2022first}, but low signal levels make clinical translation difficult, because of this current attempts rely on point scanning systems~\cite{weyers2022intraoperative,noble2023intraoperative} that will inherently limit system resolution or require slow capture times so may not be suitable for all surgery types. The main goal of our work is to relax the difficult contrast agent constraints and increase the span of viable agents by making better use of low signal data through computational video denoising. 

